Wave Tracing: Generalizing The Path Integral To Wave Optics

Modeling the wave nature of light and the propagation and diffraction of electromagnetic fields is crucial for the accurate simulation of many phenomena, yet wave simulations are significantly more computationally complex than classical ray-based models. In this work, we start by analyzing the classical path integral formulation of light transport and rigorously study which wave-optical phenomena can be reproduced by it. We then introduce a bilinear path integral generalization for wave-optical light transport that models the wave interference between paths. This formulation subsumes many existing methods that rely on shooting-bouncing rays or UTD-based diffractions, and serves to give insight into the challenges of such approaches and the difficulty of sampling good paths in a bilinear setting. With this foundation, we develop a weakly-local path integral based on region-to-region transport using elliptical cones that allows sampling individual paths that still model wave effects accurately. As with the classic path integral form of the light transport equation, our path integral makes it possible to derive a variety of practical transport algorithms. We present a complete system for wave tracing with elliptical cones, with applications in light transport for rendering and efficient simulation of long-wavelength radiation propagation and diffraction in complex environments.

==> results.tex <==
\begin{figure*}[tb]
    \centering

    \begin{subfigure}[t]{1\linewidth}
        \centering
        \begin{adjustbox}{width=\linewidth}
            \inputtikz{results1}
        \end{adjustbox}
        \caption{
            Signal coverage simulations in realistic city scenes (from \citet{sionna}), done in full 3D.
            Visualized is the received signal strength in decibels that reaches the street level.
            Emitter position is marked with a red-yellow circle.
            Simulation is done using (left) pure ray tracing with no diffractions; or with with UTD-based diffractions using a (middle) 30GHz or (right) 1GHz carrier.
            % Note the difference in rss over the shadowed streets and areas.
            Buildings' surfaces are perfectly-specular materials with different refractive indices.
        }
        \label{fig:render_signal_coverage}
    \end{subfigure}%
    \vspace*{2.5mm}
    \hfill
    % Room
    \begin{subfigure}[t]{1\linewidth}
        \centering
        \begin{adjustbox}{width=\linewidth}
            \inputtikz{results2}
        \end{adjustbox}
        \caption{
            A metal screen is placed between a powerful collimated light source and a wall.
            A geometric aperture is cut in the middle of the screen: (left) star shaped or (right) vertical double slits.
            Our simulation reproduces the expected diffraction pattern.
            To make the light transport more challenging we place a (left) mirror or (right) dielectric bunny, making direct sampling techniques difficult.
            This shows that we able to importance sample the entire multi-edge diffraction well.
        }
        \label{fig:render_room}
    \end{subfigure}%
    \vspace*{-2mm}

    \caption{}
    \label{fig:results}
\end{figure*}

